Differentially Private Algorithms for Statistical Verification of Cyber-Physical Systems

Statistical model checking is a class of sequential algorithms that can verify specifications of interest on an ensemble of cyber-physical systems (e.g., whether 99% of cars from a batch meet a requirement on their energy efficiency). These algorithms infer the probability that given specifications are satisfied by the systems with provable statistical guarantees by drawing sufficient numbers of independent and identically distributed samples. During the process of statistical model checking, the values of the samples (e.g., a user's car energy efficiency) may be inferred by intruders, causing privacy concerns in consumer-level applications (e.g., automobiles and medical devices). This paper addresses the privacy of statistical model checking algorithms from the point of view of differential privacy. These algorithms are sequential, drawing samples until a condition on their values is met. We show that revealing the number of the samples drawn can violate privacy. We also show that the standard exponential mechanism that randomizes the output of an algorithm to achieve differential privacy fails to do so in the context of sequential algorithms. Instead, we relax the conservative requirement in differential privacy that the sensitivity of the output of the algorithm should be bounded to any perturbation for any data set. We propose a new notion of differential privacy which we call expected differential privacy. Then, we propose a novel expected sensitivity analysis for the sequential algorithm and proposed a corresponding exponential mechanism that randomizes the termination time to achieve the expected differential privacy. We apply the proposed mechanism to statistical model checking algorithms to preserve the privacy of the samples they draw. The utility of the proposed algorithm is demonstrated in a case study.

==> backup.tex <==
Specifically, the functionality specifications are mathematically expressed by formal languages (e.g., temporal logics), and the statistical model checker

the research on differential privacy has flourished during the past decade~\cite{dwork2013algorithmic} and has been applied extensively to various statistical inference, learning, and optimization problems~\cite{kusner2015differentially,huang2014cost,jain2013differentially,rogers2016maxinformation,wang2017differential}. Differentially private probably approximately correct (PAC) learning is based on a body of literature established during the past decade; see for instance~\cite{kasiviswanathan2011what,blum2013learning} and references therein.


When it holds, as the number of samples increases, the samples will be increasingly concentrated on one side of p by the central limit theorem. Therefore, a statistical analysis based on the majority of the samples has an increasing accuracy. When is violated, the samples would be evenly distributed on the two sides of p, regardless of the sample size. Thus, no matter how the sample size increases, the accuracy of any statistical test would not increase. This will be illustrated later in the proof of Theorem.


\section{Problem Formulation}

We consider the differential privacy of a general sequential algorithm $\mathscr{A}$. The input algorithm is an (infinite) sequence of independent and identically distributed (i.i.d.) sample data $X=X_{1}, X_{2}, \ldots$ referred to as a data sequence, from some probability space $(\Omega, \Sigma, P)$. Let $\Omega^{*}=\Omega \cup(\Omega \times \Omega) \cup \ldots$ be the set of finite sequences taken from $\Omega$. Then, a sequential algorithm is defined as a tuple $\mathscr{A}=\left(T_{\mathscr{A}}, f_{\mathscr{A}}\right)$, where

\begin{itemize}
  \item $T_{\mathscr{A}}: \Omega^{*} \rightarrow\{0,1\}$ is a stopping condition, where 0 and 1 stand for false and true, respectively;

  \item $f_{\mathscr{A}}: \Omega^{*} \rightarrow \mathscr{O}$ is a return function, where $\mathscr{O}$ is the set of outputs of the algorithm $\mathscr{A}$. The set $\mathscr{O}$ can be of general type, such as binary or real numbers $\mathbb{R}$.
\end{itemize}

The sequential algorithm $\mathscr{A}$ executes on a data sequence $X$ as follows. Iteratively for $n=1,2, \ldots$ if $\tau\left(X_{1}, \ldots, X_{n}\right)=1$, then $\mathscr{A}$ stops and returns $T_{\mathscr{A}}\left(X_{1}, \ldots, X_{n}\right)$; otherwise, it continues.

The number of iterations $\mathscr{A}$ executed on the data sequence $X$ is denoted by $\tau_{\mathscr{A}}$ and is referred to as the stopping step. Mathematically, $\tau_{\mathscr{A}}$ is a stopping time [21] defined on the random process $X$, so we may also write it as $\tau_{\mathscr{A}}(X)$. Below, we introduce two examples of sequential algorithms.




  

This assertion $\mathcal{A}$ becomes more accurate in terms of decreasing $\alpha_\textrm{FP}$ and $\alpha_\textrm{FN}$ when the number of samples $N$ increases. 
\begin{assumption} \label{as:indifference_2}
There exists a known indifference parameter $\delta > 0$ such that $|p_{\varphi, f} - p| > \delta$ in the statement~\eqref{eq:problem 2}.
\end{assumption}

Consider a risk minimization problem of 
\begin{equation} \label{eq:rm}
R = \min_{f \in \mathcal{F}} \int_{\Omega} f \d P,	
\end{equation}
where $P$ is an unknown probability distribution on a set $\Omega$ and $\mathcal{F}$ is a (possibly infinite) set of integrable functions on $\Omega$. 


Since the distribution $P$ is unknown, the minimum in~\eqref{eq:erm} cannot be found by integration. To solve it empirically, we take a set of random sample points 
$$x_{1:N} = (x_1, \ldots, x_N)$$ 
from the set $\Omega$ using the unknown distribution $P$. Then, the empirical average $\sum_{i \in [N]} f(x_i) / N$ is an unbiased estimator that converges to $\int_{\Omega} f \d P$ for each $f$, as $N \to \infty$. Thus, we expect to solve the risk minimization problem~\eqref{eq:erm} by solving the empirical risk minimization problem
\begin{equation} \label{eq:erm}
R_{x_{1:N}} = \min_{f \in \mathcal{F}} \frac{\sum_{i \in [N]} f(x_i)}{N}.
\end{equation}


The statistical error of approximating~\eqref{eq:rm} with~\eqref{eq:erm} can be captured by the empirical Rademacher average over the sample points $x_{1:N}$
\begin{equation} \label{eq:era}
\gamma_{\mathcal{F}} (x_{1:N}) = \frac{\max_{f \in \mathcal{F}} \big| \sum_{i=1}^{N} \eta_i f(x_i) \big|}{N},
\end{equation}
where $\eta_{1}, \ldots, \eta_{n}$ are i.i.d. Rademacher random variables with probability distribution 
$$
\eta_i = \begin{cases}
1, & \text{with probability } 0.5, \\
-1, & \text{with probability } 0.5.
\end{cases}
$$
By Theorem 1 of~\cite{koltchinskii2000improved}, when the conditions 
\begin{equation} \label{eq:condition}
\begin{split}
& \gamma_{\mathcal{F}} (x_{1:N}) < \frac{\beta}{5},
\\ & N > \frac{4}{\beta^2} \ln \big( \frac{4}{\alpha} \big) 	
\end{split}
\end{equation}
holds for some $\alpha, \beta > 0$, we have 
\begin{equation} \label{eq:bounds}
	\mathbb{P}_{x_1, \ldots, x_N \sim P} \big( |R - R_{x_{1:N}}| < \beta \big) > 1 - \alpha,
\end{equation}
holds for any probability distribution $P$ and $R$, $R_{x_{1:N}}$ defined by~\eqref{eq:rm}\eqref{eq:erm}, respectively.


The above results build a confidence interval of the minimal risk $R$ in~\eqref{eq:erm}. By combining\eqref{eq:era}\eqref{eq:condition}\eqref{eq:bounds}, we have  
\begin{equation} \label{eq:confidence interval}
\begin{split}
& R \in \Big( \frac{\min_{f \in \mathcal{F}} \sum_{i \in [N]} f(x_i)}{N} - \frac{5 \max_{f \in \mathcal{F}} \big| \sum_{i=1}^{N} \eta_i f(x_i) \big|}{N}, \\
& \qquad \frac{\min_{f \in \mathcal{F}} \sum_{i \in [N]} f(x_i)}{N} + \frac{5 \max_{f \in \mathcal{F}} \big| \sum_{i=1}^{N} \eta_i f(x_i) \big|}{N} \Big)
\end{split}
\end{equation}
with significance level $\alpha$, i.e., with probability at least $1 - \alpha$.


where $\underline{p}_N$ is defined by~\eqref{eq:underline p}

Generally, the algorithm $\mathscr{A}$ is differentially private, if the value of the data sequence $\sigma$ cannot be easily inferred from the random public observations $\left(\tau_{\mathscr{A}}(\sigma), o_{\mathscr{A}}\left(\sigma_{1}, \ldots, \sigma_{\tau_{\mathscr{A}}}\right)\right)$. 





Differential privacy requires for any two adjacent data sequences $\sigma$ and $\sigma^{\prime}$, the probability distributions of the two (random) public observations $\left(\tau_{\mathscr{A}}(\sigma), o_{\mathscr{A}}\left(\sigma_{1}, \ldots, \sigma_{\tau_{\mathscr{A}}}\right)\right)$ and $\left(\tau_{\mathscr{A}}\left(\sigma^{\prime}\right), o_{\mathscr{A}}\left(\sigma_{1}^{\prime}, \ldots, \sigma_{\tau_{\mathscr{A}}}^{\prime}\right)\right)$ should be similar enough to satisfy the following inequality.


It is easy to check that neither of the two example sequential algorithms is differentially private.




% Following Section II-B we design a weakly differentially private sequential probability ratio test by first randomizing the stopping condition. The sequential empirical risk minimization algorithm is already random due to Rademacher random variables. This automatically gives a degree of privacy.

% To begin with, we consider the stopping step. For any $f \in \mathscr{F}$, we note that $f\left(\sigma_{i}\right)$ obeys Bernoulli distribution with parameter $P(f)$. For Rademacher random variables $\sigma_{i}$, we have
% $$
% \frac{1}{\sqrt{n}} \sum_{i=1}^{n} \sigma_{i} f\left(\sigma_{i}\right) \rightarrow \operatorname{Gaussian}(0, P(f)), \quad n \rightarrow \infty
% $$
% by Central Limit Theorem. Consequently, we have
% $$
% \frac{1}{\sqrt{n}} \sup _{f \in \mathscr{F}}\left|\sum_{i=1}^{n} \sigma_{i} f\left(\sigma_{i}\right)\right| \rightarrow|\operatorname{Gaussian}(0, \lambda)|, \quad n \rightarrow \infty
% $$
% where $\lambda=\sup _{f \in \mathscr{F}} P(f)$, as the process with the largest $P(f)$ will dominate as $n \rightarrow \infty$.

% The probability of terminating at $N_{\alpha, \beta}$ is
% $$
% \begin{aligned}
% \mathbb{P}[\tau&=N_{\alpha, \beta]}=\int_{0}^{\alpha N_{\alpha, \beta}} \sqrt{\frac{2}{\lambda \pi N_{\alpha, \beta}}} e^{-\frac{x^{2}}{2 \lambda N_{\alpha, \beta}}} \mathrm{d} x \\
% & \approx \sqrt{\frac{2 \lambda}{\alpha^{2} \pi N_{\alpha, \beta}}} e^{-\frac{\alpha^{2} N_{\alpha, \beta}}{2 \lambda}}
% \end{aligned}
% $$
% Thus, the log-likelihood ration of two adjacent input sequences with $f\left(\sigma_{1}\right)=0$ and $f\left(\sigma_{1}^{\prime}\right)=1$ satisfies
% $$
% \begin{aligned}
% &\ln \frac{\mathbb{P}\left[\tau \mid f\left(\sigma_{1}\right)=1\right]}{\mathbb{P}\left[\tau \mid f\left(\sigma_{1}\right)=0\right]}\\
% &=\ln \frac{\int_{0}^{\alpha N_{\alpha, \beta}-1} \sqrt{\frac{2}{\lambda \pi\left(N_{\alpha, \beta}-1\right)}} e^{-\frac{x^{2}}{2 \lambda\left(N_{\alpha, \beta}-1\right)}} \mathrm{d} x}{\int_{0}^{\alpha N_{\alpha, \beta}} \sqrt{\frac{2}{\lambda \pi\left(N_{\alpha, \beta}-1\right)}} e^{-\frac{x^{2}}{2 \lambda\left(N_{\alpha, \beta}^{2}-1\right.} \mathrm{d} x}}\\
% &\approx \sqrt{\frac{2}{\lambda \pi N_{\alpha, \beta}}} e^{-\frac{\alpha^{2} N_{\alpha, \beta}}{2 \lambda}},
% \end{aligned}
% $$
% noting that $\alpha N_{\alpha, \beta} \gg 1$ for $\alpha \ll 1$.

% The probability of terminating at step $\tau+N_{\alpha, \beta}$ satisfies asymptotically,
% $$
% \begin{gathered}
% \mathbb{P}\left[\tau=N_{\alpha, \beta}\right]=\int_{0}^{\infty} \frac{\pi x}{\lambda} \sqrt{\frac{1}{(1-\lambda) \tau^{3} N_{\alpha, \beta}}} e^{-\frac{\left(\alpha N_{\alpha, \beta}+x\right)^{2}}{2 \lambda N_{\alpha, \beta}}} \\
% e^{-\frac{(x-\alpha \tau)^{2}}{2 \pi(1-\lambda)}} \mathrm{d} x
% \end{gathered}
% $$
% where the second exponential comes from an inverse Gaussian distribution describing first hitting. Again, the loglikelihood ration of two adjacent input sequences with $f\left(\sigma_{1}\right)=0$ and $f\left(\sigma_{1}^{\prime}\right)=1$ satisfies
% $$
% \ln \frac{\mathbb{P}\left[\tau=N_{\alpha, \beta} \mid f\left(\sigma_{1}\right)=1\right]}{\mathbb{P}\left[\tau=N_{\alpha, \beta} \mid f\left(\sigma_{1}\right)=0\right]} \approx \sqrt{\frac{2 \lambda}{\alpha^{2} \pi N_{\alpha, \beta}}} e^{-\frac{\alpha^{2} N_{\alpha, \beta}}{2 \lambda}}
% $$
% By 23 and 23 , we know that the randomness in the sequential learning algorithm gives the algorithm some level of expected differential privacy.

% The return function $o_\mathscr{A} $ can be randomized by the exponential randomization algorithm proposed [8], [9] with any $\varepsilon$. Then the overall privacy level will be $\max \{\varepsilon$, $\left.\sqrt{2 / \lambda \pi N_{\alpha, \beta}} e^{-\alpha^{2} N_{\alpha, \beta} / 2 \lambda} \max \{1, \lambda / \alpha\}\right\}$. The above discussions are summarized by Algorithm 2 and Theorem 2


% Theorem 2: Algorithm 2 is $\max \left\{\varepsilon, e^{-\alpha^{2} N_{\alpha, \beta} / 2 \lambda} \max \{1\right.$, $\left.\lambda / \alpha\} \sqrt{2 / \lambda \pi N_{\alpha, \beta}}\right\}$-weakly differentially private.

% In Algorithm 2 only the return function is randomized, therefore its sample efficiency is still the same as the nonprivate version. The accuracy of the algorithm will decrease in the same way as non-sequential empirical risk minimization [24], so the discussion is omitted.



\begin{lemma} \label{lem:exponential mechanism 2}
  For a sequential algorithm $\mathscr{A}$ with a deterministic termination time $\tau_\mathscr{A}$, consider another sequential algorithm $\mathscr{B}$ with the same input and output spaces as $\mathscr{A}$ and with a random termination time $\tau_{\mathscr{B}}$ that satisfies
  \begin{equation} \label{eq:exponential mechanism 2}
  \mathbb{P}_{\mathscr{B}} \big( \mathbb{E}_{\sigma_{1:\infty}} \big[ \tau_\mathscr{B} (\sigma_{1:\infty}) = k \big] \big) 
  = \frac{e^{- \varepsilon |k - \tau_\mathscr{A} (\sigma_{1:\infty})| / \Delta_{\tau_\mathscr{A}}}}{\sum_{h \in \nat} e^{- \varepsilon |h - \tau_\mathscr{A} (\sigma_{1:\infty})| / \Delta_{\tau_\mathscr{A}}}},
  \end{equation}
  where $\sigma_{1:\infty}$ is a random sequence of signals obeying the distribution of the probabilistic model $\mathcal{S}$. Then,  $\mathscr{B}$ achieves $2 \varepsilon$-expected differential privacy. 
  \end{lemma}
  
  \begin{proof}
  % Our proof is similar to the proof of Lemma~\ref{lem:equivalence}. 
  When the significance level $\alpha \to 0$, we have $\tau_\mathscr{A} (\sigma_{1:\infty}), \tau_\mathscr{A} (\sigma_{1:\infty}') \to \infty$. 
  By the law of large numbers, equations~\eqref{eq:expected sensitivity} and~\eqref{eq:exponential mechanism 2} imply that
  $$
  \mathbb{P}_{\sigma_{-n}} \Big( 
  \big| \tau_\mathscr{A} (\sigma_{1:\infty}) - \tau_\mathscr{A} (\sigma_{1:\infty}') \big| \leq \Delta_{\tau_\mathscr{A}}
  \Big) \to 1.
  $$
  for any pair of signals $\sigma_n$ and $\sigma'_n$, 
  where $\sigma_{-n}$ is a random sequence of signals obeying the distribution of the probabilistic model $\mathcal{S}$ and $\sigma'_{-n} = \sigma_{-n}$.
  %, as $\tau_\mathscr{A} (\sigma_{1:\infty}), \tau_\mathscr{A} (\sigma_{1:\infty}') \to \infty$.
  
  By the triangle inequality, it implies that for any $k \in \mathbb{N}$,
  $$
  \mathbb{P}_{\sigma_{-n}} \Big( 
  \big| \tau_\mathscr{A} (\sigma_{1:\infty}) - k \big| - \big| \tau'_\mathscr{A} (\sigma_{1:\infty}) - k \big| \leq \Delta_{\tau_\mathscr{A}}
  \Big) \to 1.
  $$
  Taking the exponential gives 
  \todo{ I think we need more steps here as well, it is not clear to say that the conditions imply that}
  \begin{equation} \label{eq:4}
  \mathbb{P}_{\sigma_{-n}} \Big( \frac{e^{- \varepsilon  |\tau_\mathscr{A} (\sigma_{1:\infty}) - k| / \Delta_{\tau_\mathscr{A}}}}{e^{- \varepsilon  |\tau_\mathscr{A} (\sigma_{1:\infty}') - k| / \Delta_{\tau_\mathscr{A}}}} \leq e^\varepsilon \Big) \to 1.
  \end{equation}
  Since~\eqref{eq:4} holds for any $k$, we have
  \begin{equation} \label{eq:5}
  \mathbb{P}_{\sigma_{-n}} \Big( \frac{\sum_{k} e^{- \varepsilon  |\tau_\mathscr{A} (\sigma_{1:\infty}) - k| / \Delta_{\tau_\mathscr{A}}}}{\sum_{k} e^{- \varepsilon |\tau_\mathscr{A} (\sigma_{1:\infty}') - k| / \Delta_{\tau_\mathscr{A}}}} \leq e^\varepsilon \Big) \to 1.
  \end{equation}
  Thus, taking the ratios of~\eqref{eq:3} and~\eqref{eq:4} gives
  \begin{equation}
  \mathbb{P}_{\sigma_{-n}} \bigg( \frac{\mathbb{P}_{\mathscr{B}} \big( \tau_{\mathscr{B}}(\sigma_{1:\infty}) = k \big)}{\mathbb{P}_{\mathscr{B}} \big( \tau_{\mathscr{B}}(\sigma_{1:\infty}') = k \big)} \leq e^{2 \varepsilon} \bigg) \to 1
  \end{equation}
  So the lemma holds. 
  \end{proof}

==> smc.tex <==
\section{Statistical Model Checking for STL Specifications with Undetermined Test Function}
\label{sec:parametrized smc}

In practice, many specifications are given with undetermined test functions. For example, suppose the $\mathcal{S}$ is an autonomous electric car and the signal $\sigma = (\sigma_1, \sigma_2)$ is the velocity and battery level. The performance specification in signal temporal logic  
\begin{equation} \label{eq:ex2}
	(f_2 (\sigma_2) > 0) \ \mathcal{U}_{[0, 10]} \ (f_1 (\sigma_1) > 0)
\end{equation}
means within a time horizon of $10$, the car velocity should maintain $f_2 (\sigma_2) > 0$ before the battery level becomes $f_1 (\sigma_1) > 0$. This specification generalizes the specification in Example~\ref{ex:1} with the undetermined test functions $f = (f_1, f_2) \in \mathcal{F}$. They are customizable and may be different from car to car. For the manufacturer, a key problem is whether the satisfaction probability of the STL specification is greater than some given probability threshold $p \in [0,1]$ for any possible choice of $f \in \mathcal{F}$. 


\subsection{STL with Undetermined Test Functions} \label{sub:stl}

Formally, let $\varphi_f$ be an STL formula with undetermined test functions $f \in \mathcal{F}$ (like in~\eqref{eq:ex2}). We typically want to reason about the minimal/maximal satisfaction probability. To simplify the discussion, we focus on checking the minimal probability of $\sigma$ satisfying $\varphi_f$ is greater than some given probability threshold $p \in [0,1]$, i.e.,
\begin{equation} \label{eq:problem 2}
	\min_{f \in \mathcal{F}} \mathbb{P}_{\sigma \sim \mathcal{S}} ( \sigma \models \varphi_f ) = \min_{f \in \mathcal{F}} p_{\varphi_f} = \underline{p} > p
\end{equation}
where $\sigma$ is a random signal drawn from the probabilistic model $\mathcal{S}$. Maximal probabilities can be handled similarly via
$$\min_{f \in \mathcal{F}} \mathbb{P}_{\sigma \sim \mathcal{S}} ( \sigma \models \varphi_f ) > p \Longleftrightarrow \min_{f \in \mathcal{F}} \mathbb{P}_{\sigma \sim \mathcal{S}} ( \sigma \models \varphi_f ) \leq 1 - p.$$

To infer the correctness of the statement~\eqref{eq:problem 1} by statistical inference, we formulate it as a hypothesis testing problem
\begin{align} \label{eq:problem 2 ht}
& H_\textrm{null}: \underline{p} > p, \notag
\\ & H_\textrm{alt}: \underline{p} \leq p, 
\end{align}
where $H_\textrm{null}$ and $H_\textrm{alt}$ are the null and alternative hypotheses. Let 
$$\sigma_{1:N} = (\sigma_1, \ldots, \sigma_N)$$ 
be independent sample signals from the probabilistic model $\mathcal{S}$ (see Remark~\ref{rem:independent}). Now to check~\eqref{eq:problem 2 ht}, we evaluate the truth value of $\varphi$ on each sample signals $\sigma_i$ by $\varphi_f(\sigma_i)$, as defined in~\eqref{eq:varphi}. Each $\varphi(\sigma_i)$ is a binary random variable with parameter $p_{\varphi_f}$. 

Since the sample signals $\sigma_{1:N}$ are independent, the sum $\sum_{i \in [N]} \varphi_f (\sigma_{i}) \sim \mathrm{Binom} (N, p_{\varphi_f})$ obeys the binomial distribution. Thus, the satisfaction probability $p_{\varphi_f}$ can be approximated by the sample average $\sum_{i \in [N]} \varphi_f ( \sigma_{i})/N$ for each $f \in \mathcal{F}$. Accordingly, the minimal satisfactions probability $\min_{f \in \mathcal{F}} p_{\varphi_f}$ can be approximated by the minimal empirical satisfactions probability
\begin{equation} \label{eq:underline p}
\underline{p}_N = \frac{\min_{f \in \mathcal{F}} \sum_{i \in [N]} \varphi_f ( \sigma_{i})}{N}.
\end{equation}
Therefore, we define the statistical assertion for the statement~\eqref{eq:problem 2 ht} as
\begin{align} \label{eq:assert_2}
& \mathscr{A} \big( \sigma_{1:N} \big) = \begin{cases}
	H_\textrm{null}, &\text{ if } \underline{p}_N > p \\
	H_\textrm{alt}, &\text{ otherwise.}
\end{cases}
\end{align}
where $\underline{p}_N$ is defined in~\eqref{eq:underline p}. 


\subsection{Empirical Risk Minimization} 
\label{sub:erm}

To facilitate further discussion, let $\Omega$ be the set of all signals, $P$ be the unknown probability distribution of the sample signals $\sigma_1, \ldots, \sigma_N$, and 
\begin{equation} \label{eq:P_N}
P_N = \frac{1}{N} \sum_{i \in [N]} \delta_{\sigma_i} 
\end{equation}
be the empirical sample distribution, where $\delta$ is the Dirac delta function. Then, with a slight abuse of notations, we can write
\begin{align}
& \underline{p} = \min_{f \in \mathcal{F}} P(f) = \min_{f \in \mathcal{F}} \int_{\Omega} \varphi_f (\sigma) \d P,	
\\ & \underline{p}_N = \min_{f \in \mathcal{F}} P_N(f) = \min_{f \in \mathcal{F}} \int_{\Omega} \varphi_f (\sigma) \d P_N.
\end{align}

To ensure the assertion $\mathscr{A}$ is asymptotically accurate, i.e., $\mathscr{A}$ agrees with the ground truth of the problem~\eqref{eq:problem 2 ht} for $N \to \infty$, we make Assumption~\ref{ass:vc} that captures the complexity of the possibly-infinite function set $\mathcal{F}$. It generally holds on function sets with a finite number of parameters. By the Glivenko-Cantelli theorem, we have $P_N \to P$ in distribution for $N \to \infty$. With Assumption~\ref{ass:vc}, it holds that that $\underline{p}_N \to \underline{p}$ (see Remark~\ref{rem:Rademacher}).
\begin{assumption} \label{ass:vc}
The set of functions $\mathcal{F}$ has finite VC dimension~\cite{vapnik2000nature}.
\end{assumption}  


For statistical model checking, we need to derive quantitative bounds of the significance level of $\mathscr{A}$, i.e., the FP and FN ratios $\alpha_\textrm{FP}$ and $\alpha_\textrm{FN}$ for a finite $N$. For this goal, we use results from empirical risk minimization to capture the error of using the empirical statistic $\underline{p}_N$ in~\eqref{eq:assert_2} to approximate $\underline{p}$ in~\eqref{eq:problem 2}. To start with, the difference $|\underline{p}_N - \underline{p}|$ is bounded by the difference between $P$ and $P_n$.

\begin{lemma} \label{lem:1}
It holds that 
$$|\underline{p}_N - \underline{p}| \leq \Vert P_N - P \Vert_\mathcal{F}$$ 
where 
$$\Vert P_N - P \Vert_\mathcal{F} = \max_{f \in \mathcal{F}} \big| \int_{\Omega} \varphi_f (\sigma) \d (P-P_N) \big|$$
\end{lemma}

\begin{proof}
Let 
\begin{align*}
& f^* = \textrm{argmin}_{f \in \mathcal{F}} P(f),
\\ & f_N^* = \textrm{argmin}_{f \in \mathcal{F}} P_N(f).
\end{align*}
Then
\begin{align*}
\underline{p}_N - \underline{p} & = P_N (f_N^*) - P (f^*) 
\\ & = (P_N (f_N^*) - P_N (f^*)) + (P_N (f^*) - P (f^*)) 
\\ & \leq P (f^*) - P (f^*) \leq \Vert P_N - P \Vert_\mathcal{F}. 
\end{align*}
noting that $P_N (f_N^*) - P_N (f^*) \leq 0$. Similarly, 
\begin{align*}
\underline{p}_N - \underline{p} & = P_N (f_N^*) - P (f^*) 
\\ & = (P_N (f_N^*) - P (f_N^*)) + (P (f_N^*) - P (f^*)) 
\\ & \geq P (f^*) - P (f^*) \geq - \Vert P_N - P \Vert_\mathcal{F}. 
\end{align*}
Thus, the lemma holds.
\end{proof}

Due to the randomness in the sample signals $\sigma_{1:N}$, the difference between $\Vert P_N - P \Vert_\mathcal{F}$ is a random variable. Its expected value can be estimated by the Rademacher average, as proved in~\cite{gine1984limit}.

\begin{lemma} \label{lem:2}
It holds that 
$$\mathbb{E}_{\sigma_{1:N}} \Vert P_N - P \Vert_\mathcal{F} \leq 2 \mathbb{E}_{\sigma_{1:N}} \mathcal{R}_N (\mathcal{F})$$ 
\begin{equation*} \label{eq:Rad}
\mathcal{R}_N (\mathcal{F}) = \mathbb{E}_{\eta_{1:N}} \max_{f \in \mathcal{F}} \Big| \frac{1}{N}\sum_{i \in [N]} \eta_i \varphi_f (\sigma_i) \Big|
\end{equation*}
where $\eta_{1}, \ldots, \eta_n$ are i.i.d. Rademacher random variables with probability distribution 
$$
\eta_i = \begin{cases}
1, & \text{with probability } 0.5, \\
-1, & \text{with probability } 0.5,
\end{cases}
$$
and $\mathcal{R}_N (\cdot)$ is the Rademacher average.
\end{lemma}


By concentration inequalities, the bound of  the difference between $\Vert P_N - P \Vert_\mathcal{F}$ is a random variable. Its expected value can be estimated by the Rademacher average.


\begin{lemma} \label{lem:3}
It holds with probability at most $e^{- \frac{2 \delta^2 N}{9}}$ that 
$$|\underline{p}_N - \underline{p}| \geq 2 \mathcal{R}_N (\mathcal{F}) + \delta.$$
\end{lemma}

\begin{proof} 
By Lemma~\ref{lem:1} and~\ref{lem:2}, we have
\begin{align*}
& \mathbb{E}_{\sigma_{1:N}} \Big( |\underline{p}_N - \underline{p}| - 2 \mathcal{R}_N (\mathcal{F}) \Big)
\\ & \qquad \leq \mathbb{E}_{\sigma_{1:N}} \Big(\Vert P_N - P \Vert_\mathcal{F} - 2 \mathcal{R}_N (\mathcal{F}) \Big)  \leq 0
\end{align*}
Now we apply McDiarmid's inequality. Consider the mapping from the sample signals $\sigma_{1:N}$ to the approximation error $|\underline{p}_N - \underline{p}| - 2 \mathcal{R}_N (\mathcal{F})$. For any two values of sample signals $\sigma_{1:N}$ and $\sigma_{1:N}'$ that differ in only one entry, it is bounded by 
\begin{align*}
& \Big| \Big(|\underline{p}_N - \underline{p}| - 2 \mathcal{R}_N (\mathcal{F}) \Big) - \Big(|\underline{p}_N' - \underline{p}| - 2 \mathcal{R}_N' (\mathcal{F}) \Big) \Big| 
\\ &  \leq \Big| |\underline{p}_N - \underline{p}| - |\underline{p}_N' - \underline{p}| \Big| + 2 \Big| \mathcal{R}_N (\mathcal{F}) - \mathcal{R}_N' (\mathcal{F}) \Big| 
\\ &  \leq \Big| \underline{p}_N - \underline{p}_N'  \Big| + 2 \Big| \mathcal{R}_N (\mathcal{F}) - \mathcal{R}_N' (\mathcal{F}) \Big| \leq \frac{3}{N}, 
\end{align*}
because
\begin{align*}
&  \Big| \underline{p}_N - \underline{p}_N'  \Big| 
\\ &  = \Big| \frac{\min_{f \in \mathcal{F}} \sum_{i \in [N]} \varphi_f ( \sigma_{i} )}{N} - \frac{\min_{f \in \mathcal{F}} \sum_{i \in [N]} \varphi_f ( \sigma_{i}' )}{N} \Big|
\\ &  \leq \Big| \min_{f \in \mathcal{F}} \frac{\sum_{i \in [N]} \varphi_f ( \sigma_{i}' )}{N} - \frac{\sum_{i \in [N]} \varphi_f ( \sigma_{i})}{N} \Big| \leq  \frac{1}{N}
\end{align*}
and 
\begin{align*}
& \Big| \mathcal{R}_N (\mathcal{F}) - \mathcal{R}_N' (\mathcal{F}) \Big| =
\\ & \Big| \mathbb{E}_{\eta_{1:N}} \max_{f \in \mathcal{F}} \big| \frac{\sum_{i \in [N]} \eta_i \varphi_f (\sigma_i)}{N}  \big| - \max_{f \in \mathcal{F}} \big| \frac{\sum_{i \in [N]} \eta_i \varphi_f (\sigma_i')}{N}  \big| \Big|
\\ &  \leq \Big| \mathbb{E}_{\eta_{1:N}} \max_{f \in \mathcal{F}} \big| \frac{\sum_{i \in [N]} \eta_i \varphi_f (\sigma_i)}{N}  \big| - \big| \frac{\sum_{i \in [N]} \eta_i \varphi_f (\sigma_i')}{N}  \big| \Big|
\\ &  \leq \Big| \mathbb{E}_{\eta_{1:N}} \max_{f \in \mathcal{F}} \big| \frac{\sum_{i \in [N]} \eta_i \varphi_f (\sigma_i)}{N}  - \frac{\sum_{i \in [N]} \eta_i \varphi_f (\sigma_i')}{N}  \big| \Big| \leq  \frac{1}{N}
\end{align*}
Thus, by McDiarmid's inequality to $|\underline{p}_N - \underline{p}| - 2 \mathcal{R}_N (\mathcal{F})$, we have 
\begin{align*}
& \mathbb{P} \big( |\underline{p}_N - \underline{p}| - 2 \mathcal{R}_N (\mathcal{F}) \geq \delta \big) \leq 
\\ & \mathbb{P} \Big( |\underline{p}_N - \underline{p}| - 2 \mathcal{R}_N (\mathcal{F}) - \mathbb{E}_{\sigma_{1:N}} \big( |\underline{p}_N - \underline{p}| - 2 \mathcal{R}_N (\mathcal{F}) \big) \geq \delta \Big) 
\\ & \leq e^{- \frac{2 \delta^2 N}{9}}.
\end{align*}
Thus, the lemma holds.
\end{proof}

\begin{remark} \label{rem:Rademacher}
When Assumption~\ref{ass:vc} holds, the Rademacher average $\mathcal{R}_N (\mathcal{F}) \to 0$ as $N \to \infty$~\cite{vapnik2000nature}. So Lemma~\eqref{lem:3} implies that $\underline{p}_N \to \underline{p}$, i.e., the assertion $\mathscr{A}$ agrees with the ground truth of the problem~\eqref{eq:problem 2 ht} almost surely.
\end{remark}




\subsection{Statistical Model Checking} 
\label{sub:smc}

We now develop a sequential algorithms for the hypotheses testing problem~\eqref{eq:problem 2 ht}. By Lemma~\ref{lem:3}, for a desired significance level $\alpha > 0$, the minimal satisfaction probability $\underline{p}$ in~\eqref{eq:problem 2 ht} is contained by the confidence interval.
\begin{equation} \label{eq:confidence interval}
\underline{p} \in \big( \underline{p}_N - d_N, \ \underline{p}_N + d_N \big),
\end{equation}
\begin{equation} \label{eq:d}
d_N = 2 \mathcal{R}_N (\mathcal{F}) + \sqrt{- \frac{9 \ln \alpha}{2 N}}
\end{equation}
where $\mathcal{R}_N (\mathcal{F})$ is given by~\eqref{eq:Rad}. Thus, if $\underline{p}_N + d_N < p$, then we can assert that 
$\min_{f \in \mathcal{F}} p_{\varphi_f} < p$ with the significance level less than $\alpha$. Similarly, if $\underline{p}_N - d_N > p$, then we can assert that $\min_{f \in \mathcal{F}} p_{\varphi_f} > p$ with the significance level less than $\alpha$. Otherwise, we keep on drawing new samples. Namely, the assertion is
\begin{equation} \label{eq:assert_2}
\mathscr{A} \big( \sigma_1, \ldots, \sigma_N \big) = \begin{cases}
H_\textrm{null}, & \text{ if } \underline{p}_N - d_N > p \\
H_\textrm{alt}, & \text{ if } \underline{p}_N + d_N < p \\
\text{continue}, & \text{ otherwise.}
\end{cases}
\end{equation}
This procedure is summarized by Algorithm~\ref{alg:2}. 

To ensure the termination and accurate of Algorithm~\ref{alg:2}, we introduce Assumption~\ref{as:indifference 2}.

\begin{assumption} \label{as:indifference 2}
It holds that $\underline{p} \neq p$ in~\eqref{eq:problem 2}.
\end{assumption}

\begin{remark} \label{lem:5}
Similar in spirit with Remark~\ref{rem:2}, by Assumption~\ref{as:indifference 2}, we do not distinguish between checking $\underline{p} > p$ or checking $\underline{p} \geq p$ in~\eqref{eq:problem 2}. In addition, the maximal satisfaction probabilities can be checked via the negation of minimal satisfaction probabilities in~\eqref{eq:problem 2}. For example, 
\begin{align*}
\max_{f \in \mathcal{F}} p_{\varphi_f} < p \ & \Longleftrightarrow \ \min_{f \in \mathcal{F}} p_{\neg \varphi_f} \geq 1 - p 
\\ & \Longleftrightarrow \ \min_{f \in \mathcal{F}} p_{\neg \varphi_f} > 1 - p.
\end{align*} 
\end{remark}

With Assumption~\ref{as:indifference 2}, the termination and accurate of Algorithm~\ref{alg:2} is ensured by Theorem~\ref{thm:1}.

\begin{algorithm}[!t]
\caption{SMC of $\min_{f \in \mathcal{F}} \mathbb{P}_{\sigma \sim \mathcal{S}} ( \sigma \models \varphi_f ) > p$.\label{alg:2}}

\begin{algorithmic}[1]
\Require System $\mathcal{S}$ and desired significance level $\alpha$.

\State $N \gets 0$.

\While{True}

\State $N \gets N + 1$

\State Draw sample signal $\sigma_N$ from $\mathcal{S}$

\State $\underline{p}_N = \frac{1}{N} \min_{f \in \mathcal{F}} \sum_{i \in [N]} \varphi_f ( \sigma_{i})$

\State $\mathcal{R}_N \gets \mathbb{E}_{\eta_{1:N}} \max_{f \in \mathcal{F}} \Big| \frac{1}{N}\sum_{i \in [N]} \eta_i \varphi_f (\sigma_i) \Big|$

\State $d_N \gets 2 \mathcal{R}_N + \sqrt{- \frac{9 \ln \alpha}{2 N}}$

\If {$\underline{p}_N - d_N > p$} Return $H_\textrm{null}$

\ElsIf {$\underline{p}_N + d_N < p$} Return $H_\textrm{alt}$

\Else \ Continue

\EndIf 

\EndWhile
\end{algorithmic}
\end{algorithm}


\begin{theorem} \label{thm:1}
When $\underline{p} \neq p$ in~\eqref{eq:problem 2}, Algorithm~\ref{alg:2} terminates with probability $1$ and its return agrees with the ground truth of~\eqref{eq:problem 2} with probability at least $1-\alpha$.
\end{theorem}

\begin{proof}
{\bf Termination.} By Remark~\ref{rem:Rademacher}, we have $\mathcal{R}_N \to 0$ and $\underline{p}_N \to \underline{p}$ as $N \to \infty$. The former implies 
$$d_N = 2 \mathcal{R}_N + \sqrt{- \frac{9 \ln \alpha}{2 N}} \to 0.$$ 
The latter implies 
$$\underline{p}_N - p \to \underline{p} - p \neq 0.$$
Thus, $d_N < |p - p_N|$, i.e., the algorithm terminates for sufficiently large $N$.   

\noindent {\bf Probabilistic Correctness.} Consider the probabilistic events 
\begin{itemize}
	\item $\mathcal{T}$: The return of Algorithm~\ref{alg:2} agrees with the ground truth. 
	\item $\mathcal{T}_N$: The assertion~\eqref{eq:assert_2} agrees with the ground truth for the $N$ iteration.
\end{itemize}
Then
$\mathbb{P} (\mathcal{T}) = \sum_{i \in \nat} \mathbb{P} (\mathcal{T}_i) \mathbb{P} (N = i)$. By construction of the significance intervals, we have $\mathbb{P} (\mathcal{T}_i) > 1 - \alpha$ for any $i \in \nat$. In addition, by {\bf Termination}, we have $\sum_{i \in \nat} \mathbb{P}(\tau = i) = 1$. Thus, $\mathbb{P}(A) \geq 1 - \alpha_d$.
\end{proof}


\begin{remark} \label{lem:related}
By allowing the undetermined test function from a possibly infinite set $\mathcal{F}$, Algorithm~\ref{alg:2} simultaneously checks a possibly infinite set of STL formulas. It generalizes most previous works that focus on single STL formulas~\cite{legay2010statistical,agha2018survey}. Comparing previous work on statistical model checking for STL formula sets~\cite{wang2020probabilistic}, this method does not require the monotonicity condition on the STL formula sets. Finally, the condition $\underline{p} \neq p$ in Theorem~\ref{thm:1} is similar in spirit with~\cite{zarei2020statistical} to ensure the termination and probabilistic correctness of the statistical model checking algorithm.
\end{remark}


% \begin{remark} \label{lem:5}
% Similar in spirit with Remark~\ref{rem:2}, by the condition $\underline{p} \neq p$ in Theorem~\ref{thm:1}, we do not distinguish between checking $\underline{p} > p$ or checking $\underline{p} \geq p$ in~\eqref{eq:problem 2}. In addition, checking maximal satisfaction probabilities

% $\underline{p} < p$ or $\underline{p} \leq p$ is equivalent to checking $p_{\neg \varphi} \geq 1 - p$ or $p_{\neg \varphi} > 1 - p$. Thus, the method for checking $p_\varphi > p$ applies to the other three cases.
% \end{remark}





